Demeter: Resource-Efficient Distributed Stream Processing under Dynamic Loads with Multi-Configuration Optimization

Distributed Stream Processing (DSP) focuses on the near real-time processing of large streams of unbounded data. To increase processing capacities, DSP systems are able to dynamically scale across a cluster of commodity nodes, ensuring a good Quality of Service despite variable workloads. However, selecting scaleout configurations which maximize resource utilization remains a challenge. This is especially true in environments where workloads change over time and node failures are all but inevitable. Furthermore, configuration parameters such as memory allocation and checkpointing intervals impact performance and resource usage as well. Sub-optimal configurations easily lead to high operational costs, poor performance, or unacceptable loss of service. In this paper, we present Demeter, a method for dynamically optimizing key DSP system configuration parameters for resource efficiency. Demeter uses Time Series Forecasting to predict future workloads and Multi-Objective Bayesian Optimization to model runtime behaviors in relation to parameter settings and workload rates. Together, these techniques allow us to determine whether or not enough is known about the predicted workload rate to proactively initiate short-lived parallel profiling runs for data gathering. Once trained, the models guide the adjustment of multiple, potentially dependent system configuration parameters ensuring optimized performance and resource usage in response to changing workload rates. Our experiments on a commodity cluster using Apache Flink demonstrate that Demeter significantly improves the operational efficiency of long-running benchmark jobs.

==> sections/02_background.tex <==

\section{Background}

This section expands upon the background related to Time Series Forecasting and Bayesian Optimization.

\subsection{Time Series Forecasting}

Time series forecasting is an important area in statistics and machine learning that deals with predicting future values of a time series based on its historical data~\cite{chatfield2000time}. 
Time series data consist of observations collected sequentially over time, and they are commonly found in various domains, such as finance, economics, environmental sciences, and computer science. 
In computer science and distributed computing, time series forecasting is often used to predict dynamic workloads, which can help optimize resource allocation and improve system performance~\cite{bodik2010characterizing}. 
Forecasting techniques for time series data range from classical statistical methods, like ARIMA (AutoRegressive Integrated Moving Average)~\cite{box2015time}, to more recent machine learning approaches, such as recurrent neural networks and Long Short-Term Memory (LSTM) networks~\cite{hochreiter1997long}. 

In this paper, we employ the ARIMA model, which is a widely-used and well-established method for linear time series forecasting. 
ARIMA models combine autoregressive, differencing, and moving average components to capture different patterns in the data, such as trends and seasonality~\cite{box2015time}. 
By selecting appropriate parameters for these components, ARIMA models can be fine-tuned to fit various types of time series data and provide accurate forecasts, including those related to dynamic workloads in distributed computing environments.
We opt for the ARIMA model due to its proficiency in short-term forecasting, particularly beneficial when working with smaller datasets, in contrast to alternative machine learning methods, which typically necessitate more extensive data to generate accurate predictions~\cite{}.

\subsection{Bayesian Optimization}

Bayesian optimization is a powerful and widely-used global optimization technique for expensive black-box functions, which has been successfully applied to various domains, including machine learning, robotics, and experimental design~\cite{brochu2010tutorial}. 
It is particularly suitable for optimizing functions that are expensive to evaluate, noisy, or have unknown gradients. 
At the core of Bayesian optimization lies the use of probabilistic models, such as Gaussian processes, to model the unknown function and to guide the search for its optimum~\cite{brochu2010tutorial, shahriari2016taking}. 
Acquisition functions are then used to balance exploration and exploitation based on the uncertainty of the model~\cite{shahriari2016taking}. 
In recent years, Bayesian optimization has gained significant attention due to its ability to efficiently optimize complex, high-dimensional functions with relatively few evaluations~\cite{shahriari2016taking}.

Multi-Objective Bayesian optimization extends the standard Bayesian optimization framework to handle multiple objectives simultaneously, making it suitable for applications where multiple conflicting criteria need to be optimized~\cite{hernandez2014predictive}. 
These approaches typically involve constructing a probabilistic model for each objective and combining the information from each model to guide the search process~\cite{hernandez2014predictive}. 
Multi-Objective Bayesian optimization has proven effective in tackling complex problems with multiple competing objectives, offering a flexible and efficient way to navigate the trade-offs between different criteria.
